MigrateLib: a tool for end-to-end Python library migration

Library migration is the process of replacing a library with a similar one in a software project. Manual library migration is time consuming and error prone, as it requires developers to understand the Application Programming Interfaces (API) of both libraries, map equivalent APIs, and perform the necessary code transformations. Due to the difficulty of the library migration process, most of the existing automated techniques and tooling stop at the API mapping stage or support a limited set of libraries and code transformations. In this paper, we develop an end-to-end solution that can automatically migrate code between any arbitrary pair of Python libraries that provide similar functionality. Due to the promising capabilities of Large Language Models (LLMs) in code generation and transformation, we use LLMs as the primary engine for migration. Before building the tool, we first study the capabilities of LLMs for library migration on a benchmark of 321 real-world library migrations. We find that LLMs can effectively perform library migration, but some post-processing steps can further improve the performance. Based on this, we develop MigrateLib, a command line application that combines the power of LLMs, static analysis, and dynamic analysis to provide accurate library migration. We evaluate MigrateLib on 717 real-world Python applications that are not from our benchmark. We find that MigrateLib can migrate 32% of the migrations with complete correctness. Of the remaining migrations, only 14% of the migration-related changes are left for developers to fix for more than half of the projects.

==> c4-llm/evaluation-unseen--approach.tex <==

% \input{tabs/unseen-migration.tex}


\section{\ref{rq:unseen} \RQUnseen}
\label{sec:rq-llm-unseen}
\subsection{\ref{rq:unseen} Approach}
All the migrations in \migbench happened prior to the known training cutoff date of the three models (Late 2023).
Therefore, there is a possibility that the LLMs are simply reciting the migrated code they have seen before (for this particular code base).
To validate whether LLMs are able to perform migrations that are not known to them, but for libraries they are aware of, 
we run an experiment with repositories that never contained the target migration and that are updated after the training cutoff dates. 
To allow validating the migration, we choose repositories with high test coverage.

We use SEART~\cite{seart} to find Python repositories that are updated on or after January 1, 2024.
We only keep repositories that have a \texttt{requirements.txt} file to allow us to set up the environment to run tests.
We clone the latest version of the repositories one by one, set up a virtual environment using the requirements file, and then run tests with coverage.
We stop after we find \UnseenReposCount repositories whose tests pass and achieve at least 95\% statement coverage. 

For each repository, we select a library listed in the requirements file and identify an analogous library that provides similar functionality through an online search. 
Overall, we choose \UnseenLibPairsCount unique library pairs, \UnseenOldLibPairsCount from \migbench and \UnseenNewLibPairsCount external to it.
This allows us to evaluate migration of unseen code, both on library pairs we have seen the models perform on before, as well as on new pairs.
To ensure that the models have never seen the expected code that uses the target library in these repositories, we traverse the commit histories of each repository and confirm that the target library never appeared in the requirements file. 
This also removes the possibility that the LLMs have previously seen an inverse migration from the target library to the source library in the repository's history.

Next, we find the code files that use the source library and thus require migration.
For each of the \UnseenReposCount repositories, we parse each file using the Python AST module to find the files that import the source library and thus require migration.
We also manually locate the API usages in those files to confirm that it does not just import the library but also uses it.
We then run the available tests to record their current status and also manually verify that the API usages of the source libraries are covered by the tests.
Finally, we migrate each of the identified files using the same prompt template we used before (\autoref{fig:prompt-mig-expermiment}).
We run the tests after the migration and compare the test results to those before the migration.

Overall, for this experiment, we have a total of \UnseenMigsCount migrations in \UnseenReposCount repositories between \UnseenLibPairsCount unique library pairs.
The repositories have between \UnseenMinFilesCount and \UnseenMaxFilesCount migration-related files (median \UnseenMedianFilesCount) and between \UnseenMinApisCount to \UnseenMaxApisCount source API usages that require migration (median \UnseenMedianApisCount).
The number of tests in the 10 repositories ranges from \UnseenMinTestsCount to \UnseenMaxTestsCount (median \UnseenMedianTestsCount), all passing before migration with 95\% or more statement coverage.






==> c4-llm/evaluation-unseen--findings.tex <==
\subsection{\ref{rq:unseen} Findings}
\label{sec:unseen-eval-findings}

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\columnwidth]{c4-llm/img/unseen-migs-passed-tests.pdf} 
    \caption{Correctness of migrations unseen by the LLMs (RQ3).}
    \mysubcaption{Asterisks (\textasteriskcentered) indicate the library pair is not in \migbench.}
    \label{fig:unseen-result}
\end{figure}
    

The migrations done by the LLMs have between \UnseenMinModifiedLines and \UnseenMaxModifiedLines lines modified per migration (median \UnseenMedianModifiedLines), confirming that the LLMs attempted to migrate the code rather than returning the same code.
\autoref{fig:unseen-result} shows the percentage of passing tests for each migration. %in \rqUnseen.
The dashed lines show the median passing tests for each model across all migrations.
\fo has the highest median passing tests (\UnseenFouroMedianPassedTests), followed by \mn (\UnseenMiniMedianPassedTests).
\lm has most of the migrations (\UnseenLlamaNoPassPercent) fail, resulting in the median passing tests of \UnseenLlamaMedianPassedTests.

\fo has \UnseenFouroAllPass fully correct migrations (i.e., all tests passing after migration) plus two more migrations having 98\% and 99\% tests passing.
\fo has only \UnseenFouroNoPass fully incorrect migrations (no tests passing after migration).
\mn follows \fo with \UnseenMiniAllPass fully correct migrations, and \UnseenMiniNoPass fully incorrect migrations.
\lm has only \UnseenLlamaAllPass fully correct migration but has two migrations having 98\% tests passing.
Overall, the relative performance of the three models follow the same trend as \rqBench and \rqTest, with \fo being the best, followed by \mn and then \lm.

We now compare \rqUnseen results with \rqBench for the \UnseenOldLibPairsCount library pairs that also appear in \migbench.
This helps us understand whether migrations between these library pairs are inherently challenging or if the LLMs did better on potentially familiar code.

\aPair{attrs}{dataclasses} and \aPair{cryptography}{pycryptodome} migrations illustrate the challenging cases in these four library pairs.
We find that these library pairs show consistent poor performance across both RQs.
\lib{attr} and \lib{dataclasses} both primarily offer decorator based APIs.
Their decorators take as input a variety of arguments, many of which have default values.
We noticed that the LLMs often fail to correctly migrate these default values, leading to incorrect migrations.
In \rqUnseen, the \aPair{attrs}{dataclasses} migration results in complete failure across all three models.
Similarly in \rqBench, only 2 out of 12 attempts for this library pair by the models are fully correct.
The \aPair{cryptography}{pycryptodome} migration completely fails for two models in \rqUnseen, and only 12 out of 45 such instances are correct in \rqBench.

In contrast, \aPair{toml}{tomlkit} and \aPair{flask}{bottle} represent two consistently easier cases, where the LLMs achieve high or perfect correctness across both RQs.
Except for one \aPair{flask}{bottle} migration where the token limit was exceed for \lm in \rqBench, all migrations in these two library pairs are at least partially correct.

Overall, this suggests that the difficulty of a migration is primarily determined by the inherent complexity of the library pairs, not by whether the migration or the target code was seen during training. Specifically, library pairs that were hard for the models in \rqUnseen were also hard in \rqBench and \rqTest, while easier pairs consistently achieved better results.


%The \pair{attrs}{dataclasses} migration is the worst performed in \rqUnseen, having all three models failing all tests.
%This library pair was also found difficult in \rqBench, where there were 4 such migrations.
%None of them were fully correct for \lm and \mn, and \fo had 2 of them correct.
%\rqTest does not include a migration between this library pair.

%The \pair{cryptography}{pycryptodome} migration is also among the worst performed migration in \rqUnseen. Here, \mn has 23\% tests passing, while the other two models completely fail it.
%\rqBench has 15 such migrations, and \lm, \mn, and \fo got 20\%, 33\%, and 33\% of them correct, respectively, which are much lower than the average results in \rqBench (\autoref{tab:bm-eval-mig-level}).
%\rqTest had 2 such migrations, one fails for all three LLMs, and the other is correct for \fo and \mn, but incorrect for \lm.

%The \pair{toml}{tomlkit} migration is much better performed in \rqUnseen, especially \mn and \fo getting all tests passing.
%\rqBench has just one such migration which \lm and \fo got correct, and \mn got \migStatusExtraChange.
%This migration is also in \rqTest, and again \lm and \fo have them fully correct and \mn has it partially correct.
%Overall, this migration is relatively easier for the LLMs in all three RQs.

%The \pair{flask}{bottle} migration is best performed migration in \rqUnseen.
%\rqBench has 4 such migrations.
%Except for one token limit exceed for \lm, 
%all the LLMs got them all either correct, partially correct, or \migStatusExtraChange.
%\rqTest does not have a migration between this library pair. 

\begin{tcolorbox}[colback=resultbg]
    \textbf{\rqUnseen:}
    Out of \UnseenReposCount unseen migrations, the LLMs fully migrated \UnseenLlamaAllPass-\UnseenFouroAllPass migrations, with \fo being the highest.
    The performance patterns are consistent with those observed in \rqBench.
\end{tcolorbox}


==> c4-llm/lst/example-fail-arg-transform/_index.tex <==
\begin{figure}[!tp]
  \centering
  %\aMig{retrying}{tenacity}{intelai/inference-model-manager}{71aff3a0}
  \begin{minipage}[t]{0.32\textwidth}
    \lstinputlisting[
      language=Python, 
      title=Before migration (\lib{retrying}), 
      xleftmargin=1em,
      firstnumber=3
      ]{c4-llm/lst/example-fail-arg-transform/0-pre.py}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[
      language=Python, 
      title=Dev's migration (\lib{tenacity}), 
      xleftmargin=1em,
      firstnumber=3
      ]{c4-llm/lst/example-fail-arg-transform/1-dev.py}
  \end{minipage} 
    \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[
      language=Python, 
      title=\mn{}'s migration (\lib{tenacity}), 
      xleftmargin=1em,
      firstnumber=3
      ]{c4-llm/lst/example-fail-arg-transform/2-mn.py}
  \end{minipage}   
  
  \caption{\mn failing in argument transformation.}
  \label{fig:example-fail-arg-transform}
\end{figure}


==> c4-llm/lst/example-param-shadow-import/_index.tex <==
\begin{figure}[!tp]
  \centering
  %\aMig{ipaddr}{ipaddress}{google/capirca}{eb768ea7}
  \begin{minipage}[t]{0.32\textwidth}
    \lstinputlisting[
      language=Python, 
      title=Before migration (\lib{ipaddr}), 
      xleftmargin=1em,
      firstnumber=4
      ]{c4-llm/lst/example-param-shadow-import/0-pre.py}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[
      language=Python, 
      title=Dev's migration (\lib{ipaddress}), 
      xleftmargin=1em,
      firstnumber=4
      ]{c4-llm/lst/example-param-shadow-import/1-dev.py}
  \end{minipage} 
    \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[
      language=Python, 
      title=\mn{}'s migration (\lib{ipaddress}), 
      xleftmargin=1em,
      firstnumber=4
      ]{c4-llm/lst/example-param-shadow-import/2-mn.py}
  \end{minipage}   
  
    \caption{Example of function parameter shadowing import name.}
    \label{fig:param-shadow-import-name}
\end{figure}


==> c4-llm/tab/model-description.tex <==

\begin{table*}[t]
    \renewcommand{\arraystretch}{1}
    \centering
    \caption{Description of the models we use in our experiment.}
    \label{tab:models}
    \tablefontsize
    %\begin{adjustbox}{width=.6\columnwidth}
    \begin{tabular}{lccc}
    \toprule
    ~                                & \llama  & \mini & \fouro  \\
    \midrule
    Used version                     & 3.1-70B-Instruct   & 2024-07-18    & 2024-08-06                \\
    Knowledge cutoff                 & December 2023      & October 2023  & October 2023                  \\    
    Model Type                       & Open-source        & Proprietary   & Proprietary           \\
    \# training parameters           & 70 billion         & No official info & No official info    \\
    Context length                   & 128K tokens        & 128K tokens   & 128K tokens                                \\
    Output limit                     &  4096 tokens \tablefootnote{Llama 3.1 has an input+output limit of 8192 tokens. Our prompt and response are approximately equal, therefore we consider the output limit to be half (4096).}      & 16,384 tokens & 16,384 tokens          \\
    Cost \tablefootnote{Cost per million input token at the time of our experiments: July and August 2024} & Free               & \$0.15 &  \$2.5 \\
    \bottomrule
    
    \end{tabular}
    %\end{adjustbox}
\end{table*}


==> c4-llm/tab/unseen-migration.tex <==
\newcommand{\newRepoOne}{\href{https://github.com/david96182/ninjemail}{david96182/ninjemail}}
\newcommand{\newRepoTwo}{\href{https://github.com/hh-h/aiohttp-swagger3}{hh-h/aiohttp-swagger3}}
\newcommand{\newRepoThree}{\href{https://github.com/funilrys/PyFunceble}{funilrys/PyFunceble}}
\newcommand{\newRepoFour}{\href{https://github.com/lamoreauxlab/srpenergy-api-client-python}{\makecell[l]{lamoreauxlab/\\srpenergy-api-client-python}}}

\newcommand{\COLSP}{\enspace~}
% Commit dates:
% 1. 2024-May-29
% 2. 2024-Sep-19
% 3. 2024-Dec-30
% 4. 2024-Mar-28

\begin{table*}[t]
    \centering
    \caption{Dataset and results of experiment on data unseen by the models (RQ3). The source and target libraries in bold are new pairs, not in \migbench.}
    \label{tab:unseen-experiment}
    \scriptsize
    %\begin{adjustbx}{width=.6\columnwidth}
    \begin{tabular}{@{}c@{\COLSP}l@{\COLSP}r@{\COLSP}l@{\COLSP}l@{\COLSP}r@{\COLSP}c@{\COLSP}c@{\COLSP}c@{}}        
    \toprule
    \multicolumn{6}{c}{~} &\multicolumn{3}{c}{Results: \# (\%) Passing tests} \\ \cmidrule{7-9} 
    \# & Repository     & Cov   & Source Lib                     & Target Lib               & \# Tests & \llama       & \mini             & \fouro\\
    \midrule
    1 & \newRepoOne     & 95\%  & toml 0.10.2                    & tomlkit 0.13.2           & 85  & 0 (0\%)            & 55 (64.7\%)       & 85 (100\%)    \\   
    2 & \newRepoTwo     & 99\%  & attrs 25.1.0                   & dataclasses 0.6.0        & 192 & Syntax error       & Runtime error     & Runtime error \\    
    3 & \newRepoThree   & 96\%  & \textbf{python-dotenv 1.0.1}   & \textbf{environs 14.1.0} & 903 & Syntax error       & Runtime error     & 902 (99.9\%)  \\
    4 & \newRepoFour    & 99\%  & \textbf{python-dateutil 2.9.0} & \textbf{arrow 1.3.0}     & 43  & 42 (97.7\%)        & 30 (69.8\%)       & 42 (97.7\%)   \\
    \bottomrule

    
    \end{tabular}
\end{table*}


==> c5-tool/lst/rename_public_api/_index.tex <==
% alpden550@encrypt-decrypt-fields__a0029320__sqlalchemy__tortoise-orm
\begin{figure*}[!tp]
  \centering
  \begin{minipage}[t]{0.325\textwidth}
    \lstinputlisting[language=Python, title=Original code, xleftmargin=1em]{c5-tool/lst/rename_public_api/0-premig.py}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.325\textwidth}
    \vspace{0pt}%
    \lstinputlisting[language=Python, title=\tool migration, xleftmargin=1em]{c5-tool/lst/rename_public_api/1-llmmig.py}
  \end{minipage}   
  \hfill
  \begin{minipage}[t]{0.325\textwidth}
    \vspace{0pt}%
    \lstinputlisting[language=Python, title=Manual fix, xleftmargin=1em]{c5-tool/lst/rename_public_api/4-manmig.py}
  \end{minipage}
  
  \caption{Example of \tool renaming a public class, and we manually fixing it back to original name in a \aPair{sqlalchemy}{tortoise-orm} migration.}
  \label{fig:tool-rename-public-api}
\end{figure*}


==> c5-tool/lst/replace-exception/_index.tex <==
% alexferl@vyper__a0a6ea7f__toml__tomli: fixed with an alternative API (Exception)
\begin{figure*}[!tp]
  \centering
  \begin{minipage}[t]{0.32\textwidth}
    \lstinputlisting[language=Python, title=Original code, xleftmargin=1em]{c5-tool/lst/replace-exception/0-premig.py}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[language=Python, title=\tool migration, xleftmargin=1em]{c5-tool/lst/replace-exception/1-llmmig.py}
  \end{minipage}   
  \hfill
  \begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}%
    \lstinputlisting[language=Python, title=Manual fix, xleftmargin=1em]{c5-tool/lst/replace-exception/4-manmig.py}
  \end{minipage}
  
  \caption{Example of manually replacing exception type in a \aPair{toml}{tomli} migration.}
  \label{fig:tool-replace-exception}
\end{figure*}


==> c5-tool/tab/correctness-example.tex <==
% create a table

\begin{table*}[t]
    \caption{Example of migration correctness calculation.}
    \def\tpass{\good{Pass}}
    \def\tfail{\bad{Fail}}
    
    \centering
    \label{tab:correctness-example}
    \tablefontsize
    \begin{tabular}{lcccc}
    \toprule
    Test case & \TestReportPre  & \TestReportLLM & \TestReportMerge & \TestReportAsync  \\
    \midrule
    Test 1    & \tpass & \tpass & \tpass & \tpass \\
    Test 2    & \tpass & \tfail & \tfail & \tfail \\
    Test 3    & \tpass & \tfail & \tfail & \tpass \\
    Test 4    & \tpass & \tfail & \tpass & \tpass \\
    Test 5    & \tfail & -      & -      & - \\
    \midrule
    \# passing  & 4 & 1 & 2 & 3 \\
    \midrule
    correctness &   & 25\% & 50\% & 75\% \\
    \bottomrule
    \end{tabular}
\end{table*}

